Model Agnostic Sample Reweighting for Out-of-Distribution Learning

Distributionally robust optimization (DRO) and invariant risk minimization (IRM) are two popular methods proposed to improve out-of-distribution (OOD) generalization performance of machine learning models. While effective for small models, it has been observed that these methods can be vulnerable to overfitting with large overparameterized models. This work proposes a principled method, \textbf{M}odel \textbf{A}gnostic sam\textbf{PL}e r\textbf{E}weighting (\textbf{MAPLE}), to effectively address OOD problem, especially in overparameterized scenarios. Our key idea is to find an effective reweighting of the training samples so that the standard empirical risk minimization training of a large model on the weighted training data leads to superior OOD generalization performance. The overfitting issue is addressed by considering a bilevel formulation to search for the sample reweighting, in which the generalization complexity depends on the search space of sample weights instead of the model size. We present theoretical analysis in linear case to prove the insensitivity of MAPLE to model size, and empirically verify its superiority in surpassing state-of-the-art methods by a large margin. Code is available at \url{https://github.com/x-zho14/MAPLE}.

==> curve.tex <==
[0.4400626651102783, 0.42007030805866996, 0.38961338763809095, 0.32812404933107775, 0.29480805134258575, 0.3098564243378479, 0.3355056629683065, 0.3533825121038957, 0.3645163186326027, 0.3696341699264945, 0.3717841024312071, 0.36984506036975867, 0.3641185762543749, 0.35569323457373236, 0.3438375038081976, 0.32264172940071206, 0.3092760845533877, 0.2970553461399485, 0.2877586108993629, 0.27759348306996035, 0.2700686146007398, 0.26715313212756747, 0.2656074436586883, 0.27103623501303836, 0.2850742264628098, 0.30294969344837974, 0.31422613620757767, 0.3268920582126258, 0.3377805813343372, 0.34017035251897304, 0.34084792928297236, 0.33661305560189086, 0.3346618561588602, 0.3285173225916057, 0.3200493386886718, 0.31902585037037773, 0.31448411198761866, 0.30007287085500184, 0.2981691323763657, 0.3054193414180523, 0.31564969672984755, 0.3295441782924248, 0.3390219804981805, 0.3414533652617606, 0.33890952461258694, 0.33155552109564396, 0.3239486778917545, 0.3100894564055612, 0.2906730503801394, 0.26677493441308825, 0.24799042765928564, 0.2253150198517895, 0.21480358349468567, 0.217679995584923, 0.23504691113910978, 0.26307829636255664, 0.2984805218988773, 0.32935217593370747, 0.3538778765829482, 0.3730163536963804, 0.3890264985155924, 0.3974685674220297, 0.4016010260284572, 0.39717401017721454, 0.38699200243641485, 0.37201142599549464, 0.35405498643322186, 0.3323163252246321, 0.31099205260384366, 0.28673794342870473, 0.26646226924806504, 0.25110976550457065, 0.2408367979599524, 0.2368587536216661, 0.23357111507234662, 0.23455569905990614, 0.23824949639261236, 0.24335789333121716, 0.25233028540092983, 0.2637612403839351, 0.2760689360542755, 0.2894925657020605, 0.30440749595093064, 0.31906685359870207, 0.3300633179199535, 0.3402916688389087, 0.34977547105396717, 0.35602759776442533, 0.3591464693770323, 0.3593018199882422, 0.35844098808968783, 0.3583727983303892, 0.3576850383465979, 0.35365678009127033, 0.3487711849941652, 0.3447747357944772, 0.3428884111577774, 0.33979171956481286, 0.33312400157282357, 0.32517347313207096, 0.32100885631532683, 0.3148563156990192, 0.31038739168818114, 0.3042761274578284, 0.29689247418978715, 0.2914008887769721, 0.28768225130402497, 0.28854921640468195, 0.28828908604360315, 0.28861120636134613, 0.2925234591241408, 0.29899366324770577, 0.3067278272573541, 0.3154041545963153, 0.32581111410978797, 0.3320483181093116, 0.3368713714252671, 0.3380062861212934, 0.33772704998433783, 0.3347186320451422, 0.33010129930887006, 0.32635336055728204, 0.3234402987855717, 0.3209850594785363, 0.3175453542651213, 0.31141440895504097, 0.30427210888210054, 0.2984790268562325, 0.29132869378496246, 0.28217071395387766, 0.27236705366654973, 0.26487100819124854, 0.2610080551684164, 0.25661126379589766, 0.2538867148951422, 0.25248555075820234, 0.25212682473996345, 0.253097566166579, 0.25650492208854886, 0.26413344982365017, 0.2683246540756965, 0.27623707257431945, 0.2874933349543651, 0.29984645532917775, 0.31223861501122585, 0.3237855362258604, 0.3343125830639954, 0.3437706703616815, 0.35190043048642344, 0.3588917122562642]
[0.4108496651717147, 0.3921845358679715, 0.3625457263373909, 0.30125627415852685, 0.26661285702195997, 0.2808406120459921, 0.3063263049192823, 0.32374515280284444, 0.33416188935405683, 0.337919161689688, 0.33823944007558127, 0.3329590689002312, 0.3218461894633813, 0.3060199539310946, 0.2837706878841096, 0.24462645729521199, 0.21814878850794295, 0.19751696698922394, 0.18230067925691618, 0.16747592023830132, 0.1562461329287471, 0.14912869629761555, 0.1429323833646421, 0.14078689093260427, 0.14491046266446359, 0.15248750691063212, 0.15373629279992998, 0.15708690528484792, 0.1594871613171058, 0.15441844775845073, 0.14882498691706086, 0.13996898869906488, 0.13398669700265742, 0.125826297019553, 0.11694541087379172, 0.11313838856456537, 0.1079025870344502, 0.09739925312923574, 0.10004737015018375, 0.11773050285072141, 0.142002302313023, 0.17535693066655278, 0.19762078435871455, 0.20372700144042144, 0.20179123152485717, 0.1936439225072098, 0.18671648616386466, 0.17333319002330771, 0.15566073407224987, 0.13667638704172663, 0.1223167200006986, 0.10672385763410865, 0.09889493627108203, 0.09847951193026783, 0.10729076868357437, 0.12608027707410943, 0.15105300157737037, 0.17316769761307646, 0.19108881769936745, 0.20532296722347929, 0.2177182815221925, 0.22337089765735538, 0.22553743408818466, 0.2206399296785578, 0.21143716314906622, 0.19936541444388334, 0.18597019256839942, 0.17098750704692167, 0.1572041952347508, 0.14230100852805863, 0.1302116723257831, 0.12111388776935601, 0.11503168121780373, 0.11390719788665297, 0.11296368521100059, 0.11553273579913889, 0.11993003247544146, 0.12521095462199164, 0.13316433475394826, 0.1428830141043537, 0.15376577606810202, 0.16537520026983227, 0.17834231911940573, 0.19139953287678943, 0.20051597793766548, 0.20918671059650396, 0.21756287784273493, 0.2223385871638175, 0.22350878253771503, 0.22141815533319542, 0.21853221340375545, 0.21677704371568068, 0.2145121100585335, 0.20908237379830538, 0.2033702298448265, 0.19862864479713682, 0.19574766204677316, 0.19203600648863556, 0.18549147250976797, 0.17853374949289932, 0.17439376721629152, 0.1689567134937965, 0.1649265587658731, 0.15972203386983785, 0.15367368233409917, 0.14905923683161923, 0.1455924928255821, 0.14711388851716592, 0.14750995038062598, 0.14835515270985664, 0.15226864421513817, 0.15910995774532827, 0.16739678824814525, 0.17697211373289126, 0.1889953006786259, 0.1960643559549804, 0.20151798632888207, 0.20244099794604284, 0.20165993255183026, 0.1976897498472124, 0.19216337216792742, 0.18783485380748244, 0.18445487443909897, 0.1816170986190779, 0.17801142518228888, 0.17204626969656509, 0.1654738761471303, 0.16027898740510832, 0.15410488593838803, 0.14652521380623051, 0.13868225585052552, 0.1327596120963408, 0.13006216788817676, 0.12692210902999262, 0.12536474987988283, 0.12502599139689782, 0.12552375416383055, 0.12726494148782388, 0.1326114011156506, 0.14356127265990806, 0.15007177034094513, 0.16133116381525917, 0.17815749481125112, 0.19714493808939054, 0.2165142931653553, 0.23453287519014177, 0.2512712248838598, 0.2663490794336889, 0.27951305631518897, 0.2908498805871311]
[0.1405664434478098, 0.1741886399203796, 0.2254942336939653, 0.3292019925268621, 0.3865302791492858, 0.36221729254717727, 0.31981898419255034, 0.29054791631833915, 0.27262334446649455, 0.26506511258711224, 0.26272978129217894, 0.26823033646852407, 0.2814334257587185, 0.30052728319353195, 0.32736248817664293, 0.3744095111882515, 0.40323749247610713, 0.42569490835014534, 0.4411549039680769, 0.45563597506442133, 0.46470563816646865, 0.46742254806531663, 0.46822138394602414, 0.46158100411939984, 0.444504295337113, 0.4226964551091139, 0.4100821085912133, 0.3953458307166745, 0.38287034523482405, 0.3810086163340241, 0.38073861061766956, 0.38504142448677947, 0.3858634245265578, 0.3917276417188237, 0.40013390419350864, 0.39927056271332634, 0.402797022079657, 0.41623015146787185, 0.41054526325380863, 0.38884859440259495, 0.3616707748116763, 0.32690892896239876, 0.30310896921419817, 0.29489071229942926, 0.29552123187783147, 0.30314522546255224, 0.3104853425167607, 0.32626835091606055, 0.3491706166388166, 0.3766830558035308, 0.39722721250231213, 0.4231523743623498, 0.4349264510982478, 0.4325501386349213, 0.4143128306838436, 0.3822773672697752, 0.34295874553046635, 0.30900625602074433, 0.2819373283217721, 0.26080192406810176, 0.24288092842947223, 0.23390332127745123, 0.22986262802506316, 0.23481445119300792, 0.2457429496939492, 0.26166543746644294, 0.2808460424799523, 0.30357558972354776, 0.32586534999294425, 0.35174839179484263, 0.37338268954927045, 0.38969284738996834, 0.40036443568880786, 0.40329968078236705, 0.4057347587348365, 0.4029129967909619, 0.3971458338451647, 0.3899436951682598, 0.3787370183239932, 0.36493382858156886, 0.3499725848487348, 0.33389795031899333, 0.3160611356506977, 0.2984682330749428, 0.28552441902292613, 0.2734590742660977, 0.2621234270037718, 0.2549792641404387, 0.25193457874541464, 0.2527301960063792, 0.2547881753692307, 0.2556466604214084, 0.2572847578271684, 0.26289435097061936, 0.2694648415029692, 0.2748498165586657, 0.27729896218422284, 0.28134964393882217, 0.2897612941603566, 0.29945742887074794, 0.3041361613644594, 0.3113010950194122, 0.3163038134038397, 0.32330324259773235, 0.3319860517455086, 0.33836864983249415, 0.3426449509656289, 0.3398222335800217, 0.33870440731199347, 0.3370080556712968, 0.33100159496330356, 0.3216287950552822, 0.31072199598386663, 0.2986097805585089, 0.2839842907036363, 0.2749631172748643, 0.26794561548943835, 0.26564535517812465, 0.2653583148001108, 0.2685955813699236, 0.2740074771467424, 0.2782705193276905, 0.2815074827597841, 0.28421827031191343, 0.2881080793876937, 0.29493835827249676, 0.3028909348451963, 0.30916955984934, 0.3173021283605657, 0.3280765620973794, 0.3396550013924101, 0.34835692999169476, 0.3521426427143126, 0.3567854355309012, 0.3592282295491687, 0.36002536546113223, 0.3597644628901217, 0.3579220803120223, 0.3523932419417408, 0.3413126003586137, 0.33475860656196393, 0.32341644839445777, 0.3072112175395633, 0.28952442694750624, 0.27199491301762596, 0.2559550074538417, 0.24136346879227882, 0.22828797415166746, 0.21694199580563653, 0.20722501106871652]
[0.008521226270197212, 0.013556775779407702, 0.022346578449018027, 0.041417564348792554, 0.05204877772113837, 0.047085649645713976, 0.03834900045769798, 0.032324446745544126, 0.028698457290895426, 0.027381596632274286, 0.027246737718363674, 0.028965565832042187, 0.03260182314902936, 0.03775959884628041, 0.04502933882311939, 0.05832237184212676, 0.06933758130269738, 0.07973272937234427, 0.08878580587564405, 0.09929473685471964, 0.10897962662937122, 0.11629567498369554, 0.12323877565693281, 0.12659582937264927, 0.1255110022968692, 0.12186626818535835, 0.12195543719356239, 0.12067521814996643, 0.11986191211373294, 0.12440257087485088, 0.12958847318229721, 0.13837644949749228, 0.14548803648938788, 0.15392873867001763, 0.1628713773411466, 0.16856524625614247, 0.17481629532923101, 0.1862977852504783, 0.19123823421964187, 0.1880015699845979, 0.1806771929670893, 0.16819000836032688, 0.1602482072174886, 0.15992887722190463, 0.16377801198472441, 0.17165537727013247, 0.178849557296041, 0.19030905311634716, 0.2044956346476018, 0.21986564171934875, 0.23246560014479972, 0.24480873781421664, 0.25137496602554876, 0.25129033297679304, 0.24334958996710493, 0.22856404050122903, 0.20750774800841337, 0.18847385500653197, 0.17309599154327338, 0.16085878127645484, 0.15037438967539318, 0.14525716635159447, 0.1429989350556537, 0.14737151406585405, 0.15582787231216605, 0.16695772209417908, 0.17912875071537257, 0.1931205927907182, 0.20593843330590333, 0.21921263988139292, 0.2299433434072918, 0.238083499336105, 0.2437670674492508, 0.24593436770931384, 0.24773047645697913, 0.24699857714650564, 0.2446745939112399, 0.24148745687853143, 0.23576826188944708, 0.22842191693014233, 0.2201925949127982, 0.21123426891048594, 0.2011890492789659, 0.191065474079659, 0.18389629798853233, 0.17706249674163693, 0.17053828376769853, 0.16665450430244605, 0.16541023868040644, 0.16654985189425708, 0.16823857633735367, 0.16920336836239333, 0.17051821184733607, 0.17436651920136786, 0.17839374365803912, 0.1817467654980885, 0.1840649646112266, 0.18682265547013427, 0.19162317973192702, 0.19683533520153554, 0.20046120159883005, 0.20488579326686623, 0.20838222219643823, 0.2126986528167423, 0.21744776282973294, 0.22117119525110288, 0.22408030490476405, 0.22451473557932503, 0.2254966156938713, 0.22602560013002151, 0.224206272209115, 0.22026749704367937, 0.2151532611383392, 0.20901396486871576, 0.2012092679970541, 0.19692420866084373, 0.19366500121476096, 0.1939074118861585, 0.19525474125316278, 0.19899614145849226, 0.20372789150368592, 0.20754126630754502, 0.21059726132337028, 0.21317961338728503, 0.2163351411648961, 0.22160099192709004, 0.22736309488801448, 0.23207244092404636, 0.23726435324629064, 0.24322749446871791, 0.24929573714884898, 0.2540124415783217, 0.2567872081942624, 0.25968117504783783, 0.2615202138686379, 0.26246306727939195, 0.26258492474150286, 0.26171540369907687, 0.2584904677742057, 0.250992709125533, 0.24684495330227824, 0.2390152695448902, 0.22713798164181567, 0.21348417963392546, 0.199252204233585, 0.18572665229987312, 0.173052767516407, 0.1615923174298903, 0.15164445907074064, 0.14303345117440036]

==> parts/backup_non_lineartheory.tex <==
\section{Linear Theory}
Consider to learn a linear function to make prediction $\hat Y$ based on $\bX$, i.e,. $\hat Y = \bX \theta$.  \ly{$H(Y|\bX_c,\bX_b) < H(Y|\bX_c)$.
naturally $\theta$ will use $\bX_b$?}
Our goal is to learn a $\theta$ that minimize the prediction loss while discarding the bias feature.
We define the Maximal Debiased Predictor as following: 
\begin{definition}[Maximal Debiased Predictor]
The Maximal Debiased Predictor $\theta^*$ is defined as $\theta^* := [\hat \theta_c; \mathbf{0}]$, where
$$
    \hat \theta_c  := \argmin_{\theta_c}  \bbE[\|  Y - \bX_c \theta_c\|^2].
$$
\end{definition}

\section{Non-Linear Theory}
\begin{definition}[Unbiased]
The re-weighted dataset $\cD_w$ is unbiased if   $H_w[Y|\bX_b, \bX_c] = H_w[Y|\bX_c]$. 
\end{definition}
\begin{definition}[Core Feature Preserving]
The re-weighted dataset $\cD_w$ is core preserving if  $H_w[y|\bX_c] = H[y|\bX_c]$. 
\end{definition}

\begin{assumption}[Strictly positive density assumption]
\label{aux_ass:strict_pos}
 $\forall y \in \cY, \bx_b \in \cX_b, \bx_c \in \cX_c$, $P(\bX_b=\bx_b, \bX_c=\bx_c, Y=y) > 0$.
\end{assumption}
% \begin{assumption}
% Intersection (by MB).
% \end{assumption}
\begin{theorem}[Existence of a Weight]
\label{aux_thm:existence_weight}
There exists a weight, such that $\cD_w$ is debiased and core preserving.
\end{theorem}
\begin{proof}
By Assumption \ref{ass:strict_pos}, there exists a weight $w'$ such that in the weighted distribution, $P_{w'}(Y,\bX_c) = P(Y,\bX_c)$ and $P_{w'}(Y,\bX_c, \bX_b)=P_{w'}(Y,\bX_c)P_{w'}(\bX_b)$.  One can easily check 
\begin{align*}
    H_w[Y|\bX_c, \bX_b ] = H_w[Y|\bX_c],
    H_w[Y|\bX_c] = H[Y|\bX_c]
\end{align*}
\end{proof}
\begin{assumption}[Identifiability of Maximal Debiased Predictor]
The Maximal Debiased Predictor is identifiable by the metric $\cM$, i.e.,
\begin{align*}
    \cM(S) <  \cM(f), \forall f \in \cF, f \neq S.
\end{align*}
\end{assumption}
\begin{assumption}[Uniqueness of ERM Solution]
Given a weight $w \in \cW$, there exists an unique $f'$ that minimize the ERM,
\begin{align*}
    \bbE_w \ell(f'(\bX), Y) <  \bbE_w \ell(f(\bX), Y), \forall f' \in \cF, f' \neq f.
\end{align*}
\end{assumption}

\begin{theorem}
[Infinity Sample Theorem]
Given infinity samples, there exists a weight $w$, such that the solution of empirical risk minimization $\hat f_w := \argmin_{f  \in \cF} \bbE_w[\ell(f([\bX_b, \bX_c]), Y)]$ is the MDP:
\begin{align*}
    \hat f_w = S
\end{align*}
\end{theorem}
\begin{proof}
By Theorem \ref{aux_thm:existence_weight}, we already know that there exists
a weight $w'$ such that  
\begin{align*}
    H_{w'}[Y|\bX_c, \bX_b ] = H_{w'}[Y|\bX_c],
    H_{w'}[Y|\bX_c] = H[Y|\bX_c]
\end{align*}
First we aim to show that $\hat f_w \in \cF$, i.e.,  there exists a $g \in \cG$, such that 
$\hat f_w([\bX_c, \bX_b]) = g(\bX_c)$. Let 
\begin{align}
    \hat g_{w} := \argmin_{g \in \cG} \bbE_{w}[\ell(g(\bX_c), Y)]]
\end{align}
Assume that $\cF$ and $\cG$ are large enough such that the losses achieves their lower bound (conditional entropy) 
\begin{align}
    \bbE_{w}[\ell(\hat g_w(\bX_c), Y)] &= H_{w}(Y|\bX_c)\\
    \bbE_{w}[\ell(\hat f_w(\bX_c, \bX_b), Y)] &= H_{w}(Y|\bX_c, \bX_b) \\
    &= H_{w}(Y|\bX_c)
\end{align}
% By the uniqueness assumption, $\hat f_w(\bX_c, \bX_b) = \hat g_w(\bX_c)$.
Because $\hat f_w$ is the minimizer of $\bbE_{w}[\ell(\hat g_w(\bX_c), Y)]$. If $\hat g_w(\bX_c) \neq \hat f_w(\bX_c, \bX_b)$, by the uniqueness assumption and consider $g$ is in the sub class of $\cF$, we have $\bbE_{w}[\ell(\hat f_w(\bX), Y)] < \bbE_{w}[\ell(\hat g_w(\bX_c), Y)]$  . This contradicts the above results that $\bbE_{w}[\ell(\hat f_w(\bX), Y)] = \bbE_{w}[\ell(\hat g_w(\bX_c), Y)]$. So $\hat f_w(\bX) = \hat g_w(\bX_c)$ and thus $\hat f_w \in \cC$.

We already show that above $\hat f_{w} \in \cC$, by the definition of $S$, we have 
\begin{align*}
    \bbE[\ell(S([\bX_c, \bX_b]), Y)] \leq  \bbE[\ell(\hat f_{w}([\bX_c, \bX_b]), Y)]
\end{align*}
At the same time, we have the following
\begin{align}
    \bbE[\ell( \hat f_{w}([\bX_c, \bX_b]), Y)] & = \bbE[\ell(\hat g_w(\bX_c), Y)] \\
    & = \min_{g \in \cG} \bbE_w[\ell(g(\bX_c), Y)] \\
    & = \min_{g \in \cG} \bbE[\ell(g(\bX_c), Y)] \\
    & \leq \bbE[\ell(S([\bX_c, \bX_b]), Y)]
\end{align}
The first equation is has been proved before. The second equation is the definition of $\hat g_w$. The third equation is due to the $P_w(\bX_c, Y)=P(\bX_c, Y)$. The fourth inequality is due to there exists a $g_S \in \cG$ such that $S([\bX_c, \bX_b]) = g_S(\bX_c)$. So by the uniqueness assumption of $S$, we have $\hat f_w = S$. 
% Then we are going to show that \begin{align*}
%     S = \hat f = \argmin_f \bbE_{w'}[f([\bX_b, \bX_c], Y)]
% \end{align*}
The second part proof is straightforward. By Assumption \ref{ass:identifibility}, for any $f \neq f^*=f_w$, we have
\begin{align}
    \label{eqn:unqiueness_of_theta_w}
    \cM(f) > \cM(f^*) = \cM(f_w).
\end{align}
We already know that $f_w$ is in the feasible solution of MAR. Eq. \eqref{eqn:unqiueness_of_theta_w} further shows that $f_w$ achieves the minimum loss of $\cM$. Putting these together, we conclude that MAR uniquely identify $\theta^*$. 
\end{proof}

Consider linear case.
\begin{theorem}[Finite Samples. Generalization Bound of Reweighting]
\todo{The key observation is that the space of reweighting is much smaller than directly optimizing the neural network. The main obstacle is that $\cM$ should have low correlation with $\ell$}
\end{theorem}

\begin{theorem}[Benefit of coreset in terms of sample complexity]
\end{theorem}
\begin{proof}
The proof follows directly from standard sparsity/boosting.
\end{proof}
The main challenge remains is that $\cL'$ and $\cL$ should be independent.


\begin{definition}[Maximal Debiased Predictor]
The Maximal Debiased Predictor $f^*$ is 
$$
    f^* := \argmin_{f \in \cC}  \bbE[\ell(f([\bX_c, \bX_b]), Y)]
$$
where
$\cC:=\{f:\exists g \in \cG,  f([\bX_c, \bX_b])=g(\bX_c)\}$. 
\end{definition}

To make the task possible, we assume the existence of  a powerful the metric  $\cM$ that can uniquely identify $f^*$. 
\begin{assumption}
\label{aux_ass:identifibility}
The Maximal Debiased Predictor $f^*$ is identifiable by the metric $\cM$, i.e.,
\begin{align*}
    \cM(f^*) <  \cM(f), \forall  f \in \cF, f \neq f^*.
\end{align*}
\end{assumption}
The Assumption \ref{ass:identifibility} is almost necessary, otherwise there will be no method that can provably learn $f^*$. \ly{explanation}
\begin{definition}[Weighting Function] Let $\cW$ be the set of weighting function that satisfies 
\begin{align*}
    \cW = \{ w: \bX \xrightarrow[]{} \bbR^{+}| \bbE[w(x)] = 1\}.
\end{align*}
\end{definition}
Then $\forall w \in \cW$, the $w$ weighted distribution is $P_w(\bX, Y) = w(\bX)P(\bX, Y)$. We use the subscript $w$ to denote the statistics measured on the weighted distribution, i.e., $\bbE_w$ and $H_w$ denote the expectation and entropy on the weighted distribution. Let $\hat \f_w$ be the solution of the weighted empirical risk minimization, $\hat f_w := \argmin_{f} \bbE_w[\|Y - f(\bX)\|^2]$. Before introducing the main theoretical results, we first pose the following assumption on the distribution density function.
\begin{assumption}[Uniqueness of ERM Solution]
Given a weight $w \in \cW$, there exists an unique $f'$ that minimize the ERM,
\begin{align*}
    \bbE_w \ell(f'(\bX), Y) <  \bbE_w \ell(f(\bX), Y), \forall f \in \cF, f \neq f'.
\end{align*}
\end{assumption}
\begin{assumption}[Strictly positive density assumption]
\label{aux_ass:strict_pos}
 $\forall y \in \cY, \bx_b \in \cX_b, \bx_c \in \cX_c$, $P(\bX_b=\bx_b, \bX_c=\bx_c, Y=y) > 0$.
\end{assumption}
Assumption \ref{ass:strict_pos} is common in existing works because there always exists uncertainty in the data  \cite{pearl1988probabilistic,strobl2016markov,xu2021stable}. 
 The following theorem shows the theoretical guarantee of MAR.
\begin{theorem}
[Identifiability] 
\label{aux_thm:Identifiability}
Given infinity samples, there exists a weight $w \in \cW$  such that 
$\hat f_w = f^*$. Further with Assumption \ref{ass:identifibility}, MAR can uniquely identify $f^*$. 
\end{theorem}
The full proof of Theorem \ref{thm:Identifiability} is included in Appendix \ref{app:proof:thm:Identifiability}. We sketch the proof as following: first, by Assumption \ref{ass:strict_pos}, there exists a weight such that $\bX_b$ is orthogonal to $(\bX_c, Y)$ while $P_w(\bX_c, Y)=P(\bX_c, Y)$. Then the weighted least square induces a solution equal to $\theta^*$. Second, by Assumption \ref{ass:identifibility}, we know $\cM(\theta^*)$ achieves the global minimum loss. Putting these together, we know that MAR uniquely identify $\theta^*$.


==> parts/method.tex <==
\section{Model Agnostic Sample Reweighting for Out-of-Distribution Learning}
\subsection{Preliminaries}\label{sec:pre}
% Consider  a set of $E$ environments  $\mathcal{E}:=\{e_1, e_2, \ldots, e_E\}$ in the sample space $\cX \times \cY$ with different joint distributions $\textup{Pr}^e(\bs{x}, \bs{y})$, where $e\in\cE$, $\cX$ and $\cY$ are the input and target spaces, respectively. Let $\cE_{tr}\subset \cE$ be the training environments and   $\cD^e:=\{(\mathbf{x}_i^e, \mathbf{y}_i^e)\}_{i=1}^{n_e}$ be the data set drawn from  $e\in \cE_{tr}$ with $n_e$ being data set size. Based on these training data sets, the problem is to learn a {\it robust} model $f(\cdot; \bw): \cX \xrightarrow[]{} \cY$, in the sense that it can predicts $\bs{y}$ well when given $\bx$ for all $e \in \cE$ including the unseen environments $\cE\setminus \cE_{tr} $, where $\bw$ is the parameters of $f$. 
Given a dataset $\cD := \{(\mathbf{x}_i, \mathbf{y}_i)\}_{i=1}^{n}$, where $(\mathbf{x}_i, \mathbf{y}_i)$ are instantiations of $(\bX, Y) \in \bbR^{d+1}$. We define the weighted empirical loss on the dataset $\cD$ as  $\mathcal{L}(\cD, \bs{\theta}; \bs{w}) := \frac{1}{n}\sum_{i=1}^{n} w_{i}\ell(f(\mathbf{x}_i; \boldsymbol{\theta}), y_i)$  $\ell(\cdot, \cdot)$ is the loss function. We take $\mathcal{L}(\cD, \bs{\theta})$ as $\mathcal{L}(\cD, \bs{\theta}; \mathbf{1})$ for abbreviation. 
\subsubsection{IRM}
IRM assumes the dataset $\cD$ is partitioned into multiple environments, i.e., $\cD = \bigcup_{e} \cD^e$. The correlation between spurious features and  labels is unstable among the environments. IRM considers the predictor $f(\cdot; \bs \theta)$ as a composite function of $\phi(\cdot; \Phi)$ and $h(\cdot; \bv)$, i.e., $f(\cdot; \bs \theta) = h(\phi(\cdot; \Phi); \bv) $, where $\bs \theta = \{\bv, \Phi\}$ are the trainable parameters. Two popular IRM methods learn $\bs \theta$ by minimizing the following losses: 
\begin{align*}
    \vspace*{-1pt}
    \cR_{\textup{IRMv1}} (\cD,\bs{\theta}):=& \sum_{e} \mathcal{L}(\cD^e, \bs{\theta})  + \lambda \| \nabla_v\mathcal{L}(\cD^e, \bs{\theta})\|^2_2,
\end{align*} 
\begin{align*}
    \vspace*{-1pt}
    \cR_{\textup{REx}} (\cD,\bs{\theta}):=& \sum_{e} \mathcal{L}(\cD^e, \bs{\theta})  + \lambda \bbV_e [ \mathcal{L}(\cD^e, \bs{\theta})].
\end{align*}
\subsubsection{DRO}
DRO aims to optimize the worst case performance in a set of distributions within a certain distance to the original training distribution. 
GroupDRO assumes to have access to the group annotations based on the spurious features and labels in the dataset $\cD$, i.e., $\cD = \bigcup_g \cD^g$. It minimizes the worst-group error in $\{\cD^g\}_g$:  
\begin{align*}
    \cR_{\textup{Group-DRO}}(\cD, \theta) :=  \max_{g} \cL(\cD^g, \theta)  
\end{align*}
If the group information is not available, conditional value at risk (CVaR), a typical method of DRO, is to minimize the worst-case loss across all distributions in a ball around the empirical distribution by the following:
\begin{align*}
    \cR_{\textup{Cvar-DRO}}(\cD, \theta) :=  \sup_{\bs w \in \cC(\alpha)} \cL(\cD, \theta; \bs w)  
\end{align*}
where $\cC(\alpha) = \{\bs{w}: 0 \preceq \bs{w}, \|\bs{w}\|_\infty \leq 1/ (\alpha n), \|\bs{w}\|_1=1\}$. 


\subsection{Bilevel Formulation of MAPLE for IRM }
\label{sect:bi-level}
Consider a training dataset $\cD_{tr}:=\{(\mathbf{x}^{tr}_i, \mathbf{y}^{tr}_i)\}_{i=1}^{n_{tr}}$, a validation dataset $\cD_{v}:=\{(\mathbf{x}^{v}_i, \mathbf{y}^{v}_i)\}_{i=1}^{n_{v}}$, both sampled from a distribution $\mathbb{P}(\bs{X}, Y)$, $\cR_{\cD}(\boldsymbol{\theta})$ to be any DRO or IRM criterion described in the Section \ref{sec:pre} evaluated on dataset $\cD$ and model parameters $\bs{\theta}$, the sample reweighting problem can be formulated into the following bilevel optimization problem:
\begin{gather}
\min_{\bs{w} \in \mathcal{C}}  \cR(\cD_{v}, \boldsymbol{\theta}^{*}(\bs{w})) , \label{ori_formulation}\\
s.t. ~\boldsymbol{\theta}^{*}(\bs{w}) \in \argmin_{\boldsymbol{\theta}} \mathcal{L}(\cD_{tr}, \bs{\theta}; \bs w) ,  \nonumber 
\end{gather}
where $f(\cdot; \bs{\theta})$ is a network with model parameters $\bs{\theta}$ trained on a reweighted dataset; $\bs{w}$ is a weight vector with length $n_{tr}$ indicating the importance of data points and $\mathcal{C} = \{\bs{w}: 0 \preceq \bs{w}, \norm{\bs{w}}_0 \leq K\}$ is the feasible set;  $K$ indicates the remaining coreset size; $f(\bs{x}; \bs{\theta})$ is a network with model parameters $\bs{\theta}$ trained on a reweighted dataset. To further reduce the search space, we impose a $L_0$ constraint on $\bs{w}$ to further reduce the search space, and the effectiveness of $L_0$ constraint will be theorectically justified in Theorem \ref{} and empirically verified in ablation study (Appendix \ref{sec:constraint}).


Due to the discrete nature of the $L_0$ constrain on $\bs{w}$, it is hard to solve the original formulation \ref{ori_formulation} directly. Inspired by previous works on model compression \cite{L0, xiao}, we relax the original formulation to be continuous. To be precise, we consider that there comes a accompanying probability indicating whether a data point is selected:

\begin{gather}
\min_{(\bs{w}, \bs{s})\in \mathcal{C'}} \displaystyle \mathbb{E}_{ p(\boldsymbol{m}|\boldsymbol{s})} ~ \cR(\cD_{v}, \boldsymbol{\theta}^{*}(\bs{w}, \bs{m})), \label{cont_formulation}\\
s.t. ~\boldsymbol{\theta}^{*}(\bs{w}, \bs{m}) \in \argmin_{\boldsymbol{\theta}^{*}(\bs{w}, \bs{m})} \mathcal{L'}(\bs{\theta}; \bs{w}, \bs{m}) \nonumber
\end{gather}
where $\mathcal{L'}(\bs{\theta}; \bs{w}, \bs{m}) := \frac{1}{n_{tr}}\sum_{i=1}^{n_{tr}} w_{i}m_{i}\ell(f(\mathbf{x}^{tr}_i; \boldsymbol{\theta}), \mathbf{y}^{tr}_i)$, $\mathcal{C'} = \{(\bs{w}, \bs{s}): 0 \preceq \bs{w}, 0 \preceq \bs{s} \preceq 1, \norm{\bs{s}}_1 \leq K\}$ is the feasible set, $m_i$ is viewed as a Bernoulli random variable with probability $s_i$ to be $1$ and $1-s_i$ to be $0$, that is training sample {}$m_i \sim \operatorname{Bern}(s_i)$, where $s_i \in [0,1]$. Assuming the variables $m_i$ are independent, then we can get the distribution function of $\boldsymbol{m}$, i.e.,  $p(\boldsymbol{m}|\boldsymbol{s}) = \Pi_{i=1}^{n} (s_i)^{m_i}(1-s_i)^{(1-m_i)}$. Thus, the coreset size can be controlled by the sum of the probabilities $s_i$, i.e.,  $\boldsymbol{1}^\top\boldsymbol{s}$, since $\mathbb{E}_{\boldsymbol{m}\sim p(\boldsymbol{m}|\boldsymbol{s})}\|\boldsymbol{m}\|_0 = \sum_{i=1}^n s_i$. Then the discrete constraint $\|\boldsymbol{m}\|_1\leq K $ in problem (\ref{ori_formulation}) can be transformed into $\boldsymbol{1}^\top \boldsymbol{s} \leq K$ with each $s_i\in [0,1]$, which is continuous and convex. We need to point out that the relaxation from Formulation \ref{ori_formulation} to Formulation \ref{cont_formulation} is tight: at the end of training, we observe that the probabilities converge to either 0 or 1 \ref{exp:tight}. 

\subsection{Optimization by Straight-through Gumbel Softmax and Truncated Back-propagation}

By continualizing the discrete optimization problem, we optimize $\bs{w}$ and $\bs{s}$ by Straight-through Gumbel Softmax to backpropagate through the expectation over probability space. Then the gradient of \bs{s} can be calculated by:
\begin{gather}
\frac{\partial \mathbb{E}_{ p(\boldsymbol{m}|\boldsymbol{s})}\cR_{\cD_{v}}(\boldsymbol{\theta}^{*}(\bs{w}, \bs{m}))}{\partial \bs{s}} = \frac{\partial \mathbb{E}_{ p(\boldsymbol{m}|\boldsymbol{s})} ~ \cR}{\partial \bs{s}}
\end{gather}
